Numerical approximation of singular Forward-Backward SDEs

In this work, we study the numerical approximation of a class of singular fully coupled forward backward stochastic differential equations. These equations have a degenerate forward component and non-smooth terminal condition. They are used, for example, in the modeling of carbon market[9] and are linked to scalar conservation law perturbed by a diffusion. Classical FBSDEs methods fail to capture the correct entropy solution to the associated quasi-linear PDE. We introduce a splitting approach that circumvent this difficulty by treating differently the numerical approximation of the diffusion part and the non-linear transport part. Under the structural condition guaranteeing the well-posedness of the singular FBSDEs [8], we show that the splitting method is convergent with a rate $1/2$. We implement the splitting scheme combining non-linear regression based on deep neural networks and conservative finite difference schemes. The numerical tests show very good results in possibly high dimensional framework.

==> notes.tex <==
%!TEX root = main.tex
\section{notes}

Note that difficulty appears in solving the FBSDEs as the terminal condition is allowed to be non-regular.
In the orginal problem, it has a jump.
\\
Since the terminal condition is increasing, the solution is a kind of (backward) rarefaction wave and so the characteristics (FBSDEs)
are actually well posed. (see the review for the case where there is no $P$)
\\
TO DO:
\\
- comprendre ce qui se passe pour le cas sans P dans la FBSDEs
\\
- EDP lorsque la condition terminale est Lipschitz : non-div form bien posée ?
=> solution almost everywhere convergence faible de $\partial_t u$ à clarifier...



==> oldstuff.tex <==


\subsubsection{OLD : Numerical results}

%\textcolor{blue}{Here, we still consider a toy model described as before. In this case, for $0\leq n\leq N$, the discrete time process $\Gamma$ verify the following  scheme \begin{align}
%&\widehat{P}^{\pi}_{t_{n+1}} = \widehat{P}^{\pi}_{t_{n}} + b(\widehat{P}^{\pi}_{t_{n}})h + \sigma(\widehat{P}^{\pi}_{t_{n}}) \Delta \widehat{W}_n \; \text{ and } \widehat{P}^\pi_0 = p\,.\\
%	&\tilde{\Gamma}_{n+1}(\widehat{P}^\pi_{t_{n+1}}) = \eta(t_n,\widehat{P}^\pi_{t_n},\tilde{\Gamma}_{n}(\widehat{P}^\pi_{t_n}),\widehat{Z}_{t_n},\Delta t,\Delta W_{t_n})
%	\end{align}
%Hence the conditional expectation $\tilde{\Gamma}_n(\widehat{P}^\pi_{t_n}) = \esp{\Gamma_{n+1} | \widehat{P}^\pi_{t_n}}$ corresponds to the optimal solution of the following minimization problem \begin{align}
%	\widehat{L}_{n}(\theta) = \mathbb{E}\Big|\Gamma_{n+1}(\widehat{P}^\pi_{t_{n+1}}) - \eta(t_n,\widehat{P}^\pi_{t_n},\tilde{\Gamma}_{n}(\widehat{P}^\pi_{t_n}),\widehat{Z}_{t_n},\Delta t,\Delta W_{t_n})\Big|^{2}
%\end{align}
%For this scheme, one can use independent neural networks, for the approximation of $\tilde{\Gamma}_n(\cdot)$ and for the approximation of $\widehat{\mathcal{Z}}_n(\cdot) = \sigma^{T}(t_n,\cdot)D_x\tilde{\Gamma}_n(\cdot)$. In other words, the parameters are divided into $\theta = (\lambda,\omega)$ and we consider independently neural networks $\mathcal{U}_n(.;\lambda)$ and $\mathcal{Z}_n(.;\omega)$.
%\\ For numerics, we apply the scheme described above, and we use a fully connected feed-forwward network with two hidden layers which corresponds to $L=2$, and $m=d+10$ neurons on each hidden layer. We choose relu function as an activation function for the hidden layers to avoid some negative solution, and the same for the output layer. And we renormalize the data before training on the data. And we use Adam optimizer inherited in TensorFlow with mini-batch = 1000, number of batch = 100, and epoch = 100 for stochastic gradient descent method.
%\\ We will present the numerics of the above model for different volatility $\sigma=0.01, 0.3, 1.0$, which show the advantages over the different probabilistic numerical methods as we described in the introduction part.
%}


\textcolor{yellow}{\paragraph{Toy model numerics}
In dimension 10, we take $J$=100, 300, 400 in the Euler scheme respectively for volatility $\sigma$ = 0.01, 0.3, 1.0, with time horizon $T$=1.0, time steps $N$=50, time steps for upwind scheme $N_{upwind}$ = 10, and initial value $p$=0. And for neural networks, we take 2 hidden layers and 5d+10 neurons for each hidden layer. We take 1000 trajectories in each mini-batch, and use data renormalization, and check validation loss every 30 iterations. And we reported the results in the following.
%\begin{figure}\label{fig neural nets d=10}
%\centering
%\subfloat[$\sigma=0.01$]{\label{a}\includegraphics[width=.3\linewidth]{Neural_upwind_sigma_001_J_300_d_10.png}}\hfill
%\subfloat[$\sigma=0.3$]{\label{b}\includegraphics[width=.3\linewidth]{Neural_upwind_sigma_03_J_300_d_10.png}}\hfill 
%\subfloat[$\sigma=1.0$]{\label{c}\includegraphics[width=.3\linewidth]{Neural_upwind_sigma_1_J_300_d_10.png}}
%\caption{Neural nets + Upwind and proxy solution with discretization of space $J=100,300,400$, dimension $d=10$}
%\end{figure}
\begin{Remark}
	Unlike for a low dimension, for a high dimension $d$, it is essential to set a  small learning rate $0.001$ in our case and increase neurons in each layers, otherwise, the deep algorithms will diverge, explode or converge to a wrong solution. Besides, to overcome the diffusion effect related to  Upwind scheme, it's necessary to increase the discretization steps $J$ when volatility $\sigma$ decreases for the purpose of a better result.
\end{Remark}
As we increase the number of space steps $J$, the error decreases and the computational cost increases. For example, it takes about 2 hours in the case $J=400$, and 1 hour in the case $J=100$.}




%
%\section{Update}
%\subsection{Variable change $u(t,p,e) = v(t,\exp{(e+(T-t)p)})$}
%Since $u$ verifies the following PDE:
%\begin{align*}
%	\partial_tu+\cL_{p}u-F(p,u)\partial_eu = 0 \textrm{ with } u(T,p,e) = 1_{e\geq \lambda} 
%\end{align*}
%Thus by using a variable change $x =\exp{(e+(T-t)p)})$, we obtain following PDE
%\begin{align*}
%	&\partial_tv-px\partial_xv-F(p,v)x\partial_xv+b(p)(T-t)x\partial_xv+\frac{1}{2}\sigma^2(p)\{(T-t)^2 x^2\partial_{xx}v+(T-t)^2x\partial_xv\} = 0 \\ &\textrm{ with } v(t,x) = 1_{x\geq \lambda}
%\end{align*}
%After simplification, we have
%\begin{align*}
%	-p\partial_tv-F(p,v)\partial_xv+b(p)(T-t)\partial_xv+\frac{1}{2}\sigma^2(p)\{(T-t)^2 x\partial_{xx}v+(T-t)^2\partial_xv\} = 0 
%\end{align*}
%For the toy model mentioned above, we have specifically
%\begin{align*}
%	-p\partial_tv-(p-v)\partial_xv+\frac{1}{2}\sigma^2\{(T-t)^2 x\partial_{xx}v+(T-t)^2\partial_xv\} = 0 
%\end{align*}

\subsection{Error analysis}
For $\sigma=0.01$
\begin{center}
 \begin{tabular}{||c c c c||} 
 \hline
 Method & Parameters & $L_{\infty}$ & $L_{1}$ \\ [0.5ex] 
 \hline\hline
 LF & $J=2000,N_{time}=20,N=10$ & 0.0428 & 0.0165 \\ 
 \hline
 Upwind & $J=500,N_{time}=20,N=10$ & 0.0581 & 0.0229 \\
 \hline
 Particles & $N_{particles}=2000,J=1000,N=5,N^{particles}_{time}=30$ & 0.0040 & 0.0009 \\
 \hline
 Particles with 1 time step & $N^{particles}_{time}=1$ & 0.0035 & 0.0011 \\
 \hline
 NN+LF & $J=2000,N_{time}=10,N=50$ & 0.0250 & 0.0055 \\
 \hline
 NN+Upwind & $J=400,N_{time}=10,N=50$ & 0.0337 & 0.0279 \\ [1ex] 
 \hline
\end{tabular}
\end{center}
For $\sigma=0.3$
\begin{center}
 \begin{tabular}{||c c c c||} 
 \hline
 Method & Parameters & $L_{\infty}$ & $L_{1}$ \\ [0.5ex] 
 \hline\hline
 LF & $J=1500,N_{time}=20,N=10$ & 0.0295 & 0.0247 \\ 
 \hline
 Upwind & $J=300,N_{time}=20,N=10$ & 0.0366 & 0.0311 \\
 \hline
 Particles & $N_{particles}=2000,J=1000,N=5,N^{particles}_{time}=30$ & 0.0215 & 0.0104 \\
 \hline
 Particles with 1 time step & $N^{particles}_{time}=1$ & 0.0180 & 0.0135 \\
 \hline
 NN+LF & $J=1000,N_{time}=10,N=50$ & 0.0250 & 0.0183 \\
 \hline
 NN+Upwind & $J=400,N_{time}=10,N=50$ & 0.0248 & 0.0167 \\ [1ex] 
 \hline
\end{tabular}
\end{center}
Concerning the time of computation, we gives an approximation by comparing different methods above with volatility $\sigma = 0.3$.
\begin{center}
 \begin{tabular}{||c c||} 
 \hline
 Method & Time \\ [0.5ex] 
 \hline\hline
 LF &  4 seconds\\ 
 \hline
 Upwind & 3 seconds\\
 \hline
 Particles & 7 seconds\\
 \hline
 Particles with 1 time step & 3.5 seconds \\
 \hline
 NN+LF & > 3 hours\\
 \hline
 NN+Upwind & 3500 seconds\\ [1ex] 
 \hline
\end{tabular}
\end{center}
For $\sigma=1.0$
\begin{center}
 \begin{tabular}{||c c c c||} 
 \hline
 Method & Parameters & $L_{\infty}$ & $L_{1}$ \\ [0.5ex] 
 \hline\hline
 LF & $J=400,N_{time}=20,N=10$ & 0.0307 & 0.06928 \\ 
 \hline
 Upwind & $J=100,N_{time}=20,N=10$ & 0.0247 & 0.0420 \\
 \hline
 Particles & $N_{particles}=2000,J=1000,N=5,N^{particles}_{time}=30$ & 0.0344 & 0.0553 \\
 \hline
 Particles with 1 time step & $N^{particles}_{time}=1$ & 0.031 & 0.0597 \\
 \hline
 NN+LF & $J=400,N_{time}=10,N=50$ & 0.0116 & 0.0116 \\
 \hline
 NN+Upwind & $J=100,N_{time}=10,N=50$ & 0.0182 & 0.0167 \\ [1ex] 
 \hline
\end{tabular}
\end{center}

\subsubsection{Time complexity for different methods}
Denoting $N$ number of time steps, and $N_s$ number of time sub-steps for transport equation,$N_p$ the number of particles, $J$ the number of space steps.\\
1. Binomial+LF Method\\
There are $\mathcal{O}(N^2)$ transport equations to resolve which corresponds $\mathcal{O}(JN_s)$ complexity. In total, the complexity is $\mathcal{O}(N^2JN_s)$\\
2. Binomial+Upwind Method\\
Same as LF method,in total, the complexity is $\mathcal{O}(N^2JN_s)$\\
3. Binomial+Particles Method\\
There are $\mathcal{O}(N^2)$ transport equations to resolve which corresponds $\mathcal{O}(N_pN_s\log N_p)$ complexity. In addition of a complexity $\mathcal{O}(JN_p)$ for valuation.In total, the complexity is $\mathcal{O}(N^2N_pN_s\log N_p)$ + $\mathcal{O}(JN_p)$\\
4. Neural nets+transport scheme\\
Denoting $N_{T} =N_{epoch}\cdot N_{batch}\cdot N_{size}$. For each training set, we have a forward-feed neural network with three hidden layers = $[d_1,d_2,d_3]$. The input size is $d$, and two outputs with respectively size of $J$ and $Jd$. Hence the time complexity of such neural network is $\mathcal{O}(dd_1+Jdd_3+\sum_{i=1}^{2}d_id_{i+1})$. Besides, the time complexity related to transport equation scheme is $\mathcal{O}(JN_s)$. In total, the  time complexity of global network is $\mathcal{O}\Big(JN_TN_s+N_T(dd_1+Jdd_3+\sum_{i=1}^{2}d_id_{i+1})\Big)$.

\newpage
\subsection{Models to use for numerical test}
and how to use them!

In the following,  $h$ is a map from $\R^d$ to $[1,2]$, it can be given e.g. by
\begin{align} \label{eq de h}
h(p) = 1 + \frac1{1+e^{-p}}
\end{align}
which is a range shift for the sigmoid function.

\vspace{2mm}
We then consider the drift of the cumulative emission process to be given by
\begin{align} \label{eq de mu}
\mu(p,y) = h(p)-y
\end{align}
as $y$ will take value in $[0,1]$ in practice, this will lead to positive $\mu$ along the solution and an upwind scheme can be used if needed.

\subsubsection{Model based on Brownian motion}
The toy model, presented above, is of course our main model. However, it poses some challenges when one wants to use it with finite differences approximation of the transport operator. We thus look for alternative models too.

\vspace{2mm}
$\bullet$ We can consider
\begin{align}\label{eq de mupos w any d}
\ud P^\ell_t = \sigma \ud W^\ell_t \text{ and } \ud E_t = \mu(\frac1{\sqrt{d}} \sum_{\ell=1}^d P^\ell_t,Y_t) \ud t
\end{align}
for $P_0=0$, the pricing function $e \mapsto v(0,0,e)$ does not depend on the dimension...
\begin{enumerate}[i)]
\item when $d=1$, the price can be computed by using an algorithm combining binomial tree+particles. This algorithm has been numerically validated on the toy model (it will be easy to argue that it converges, the precise rate of convergence will be the topic of a subsequent work)
\item when $d=10$, one can use NN+LF and NN+upwind (since $\mu$ has always the same sign). The numerical results can be checked then against the model with $d=1$
\end{enumerate}

\vspace{2mm}
$\bullet$ However, we can consider other models based on Brownian motion that can be easily computed in low dimension (for us here, $d=1$). Indeed, models given by
\begin{align}
P_t = f(t,B_t) \text{ and } \ud E_t = \tilde{\mu}(P_t,Y_t) \ud t
\end{align}
can be computed in dimension one using BinTree+Particles as $P$ is just a function of the value of $W$ built on a recombining tree.
\\
Here, I consider function $\tilde{\mu}$ given by
\begin{align*}
\tilde{\mu}(p^1,\dots,p^\ell,y)= \left(\prod_{\ell=1}^d p^\ell \right)^{\frac1{\sqrt{d}}}e^{-\theta y}
\end{align*}
This allows us to consider the following model:
\begin{align}
\ud P^\ell_t = \mu P^\ell_t \ud t + \sigma P^\ell_t \ud W^\ell_t, \,P^\ell_0=1, \text{ and } \ud E_t = \tilde \mu(P_t,Y_t) \ud t
\end{align}
This can be computed for $d=10$ using NN+upwind (as the cum. emission drift  $\tilde{\mu}$ is always positive). Use an euler scheme for $P$  and its closed form (as a function of BM) to see the effect of the discrete time error coming from the diffusion approximation
\\
The price can be checked against the one dimension model given by
$$
P_t = f(t,B_t) = e^{\sqrt{d}(\mu-\frac{\sigma^2}{2})t+\sigma B_t} \text{ and }\ud E_t =  \tilde \mu(P_t,Y_t) \ud t
$$
(already computed I think)



==> splitting.tex <==
\section{Splitting}

\subsection{Duhamel like formulae}

We denote by $P_{s,t}$ the operator over measurable functions defined over $[0,T]\times \R$
$$P_{s,t}[\psi](s,x) = \esp{\phi(t,X^{s,x}_t)}$$
If $g:\R \mapsto \R$ then $P_{s,t}[g](s,x) = \esp{g(X^{s,x}_t)}$ simply, and in the case of $X=W$ BM (homogeneous case) $P_{s,t}g(x) = P_{t-s}g(x)=\esp{g(X^{0,x}_{t-s})}$ where $P$ is a semi-group and
\begin{align*}
\lim_{h \rightarrow 0} \frac{P_{h}g(x)-x}{h} = Ag
\end{align*}
for $g \in \cC^2$.
\\
We now apply Ito's formula to $v(t,X_t,e)$ to get
\begin{align}
\esp{v(h,X_h,e)} &= v(0,x,e) + \int_0^h\esp{\partial_t v(s,X_s,e) + \frac12\partial_{xx}v(s,X_s,e) } \ud s 
\\
&= v(0,x,e) + \int_0^h\esp{f(v(s,X_s,e)) \partial_e v(s,X_s,e)} \ud s
\\
&=v(0,x,e) + \int_0^h\esp{ \partial_e F(v(s,X_s,e))} \ud s
\\
&=v(0,x,e) + \int_0^h \partial_e \esp{F(v(s,X_s,e))} \ud s
\end{align}
Note that there is a semi-group (backward) associated to the PDE and we denote $\cS(h)g=v(0,\cdot)$ with terminal condition at $h$ equal to $g$ so that $\cS(2h)g = \cS(h)\circ \cS(h)g$.
With this notation, we have
\begin{align}
\cS(h)g& = P(h)g-\int_0^hP(s)\circ T[v(s,\cdot)] \ud s
\\
&= P(h)g-\int_0^hP(s)\circ T[\cS(h-s)g] \ud s
\end{align}
where for a smooth enough function $T[\phi] = f(\phi)\partial_e \phi = \partial_e[F(\phi)]$.
\\
We also have (Duhamel formula)
\begin{align}
\cS(h)g& = P(h)g-\int_0^h\partial_e[P(s)[F(v(s,\cdot))]\ud s
\\
& = P(h)g-\int_0^h\partial_e[P(s)[F(\cS(h-s)g)]\ud s
\end{align}
The transport semi-group  associated to $T$ is given by $\cT(h)g = u(0,\cdot)$ with $u$ solution to
\begin{align}
\partial_t u + T[u] = 0 \text{ and } u(h,\cdot) = g
\end{align}
i.e. 
\begin{align}
\cT(h)g=u(0,e) = g(e) - \int_{0}^hT[\cT(h-s)g](e)\ud s=0
\end{align}
also
\begin{align}
\cT(h)g= g(e) - \int_{0}^h\partial_e[ F(\cT(h-s)g)](e)\ud s=0
\end{align}
\subsubsection{The first Lie splitting $\cL$} is defined by
\begin{align}
\cL(h) := P(h)\circ \cT(h)
\end{align}
so that
\begin{align}
\cL(h)g &= P(h)[g - \int_{0}^h\partial_e[ F(\cT(h-s)g)](e)\ud s]
\\
&=P(h)g - \int_{0}^h\partial_e[P(h)[F(\cT(h-s)g)]](e)\ud s
\\
&=P(h)g - \int_{0}^hP(s)\partial_e[P(h-s)[F(\cT(h-s)g)]](e)\ud s
\\
&= P(h)g - \int_{0}^hP(s)\partial_e[F(\cL(h-s)g)](e) \ud s + \int_{0}^hP(s)\eta(h-s)(e)\ud s
\end{align}
with
\begin{align}
\eta(h-s)(e):=\partial_e[P(h-s)[F(\cT(h-s)g)]](e)-\partial_e[F(P(h-s)\circ \cT(h-s)g)]
\end{align}
\subsubsection{Second Lie Splitting}
\begin{align}
\hat{\cL}(h) = \cT(h)\circ P(h)
\end{align}
Observe that
\begin{align}
P(h)g= g - \int_0^hA[P(h-s)g]\ud s
\end{align}
Another Duhamel formula ? Not really because asymetry
Define (if possible...)
\begin{align}
\ud \tilde{E}^{0,p,e}_t = - f(\tilde{v}(t,p,E^{0,p,e}_t)) \ud t
\end{align}
where $\tilde{v}(0,p,e)= \cT(h)g$.\\
\begin{bluetext}
One computes:
\begin{align}
v(h,p,\tilde{E}^{0,p,e}_h) &= v(0,p,e) + \int_0^h \partial_s v(s,p,\tilde{E}^{0,p,e}_s) - f(\tilde{v}(s,p,\tilde{E}^{0,p,e}_s))\partial_e v(s,p,\tilde{E}^{0,p,e}_s)\ud s
\\
&=
v(0,p,e) + \int_0^h\left( \set{f(v(s,p,\tilde{E}^{0,p,e}_s))-f(\tilde{v}(s,p,\tilde{E}^{0,p,e}_s))}\partial_e v(s,p,\tilde{E}^{0,p,e}_s) - Av(s,p,\tilde{E}^{0,p,e}_s) \right)\ud s
\end{align}
\end{bluetext}


==> trash.tex <==
\section{old - trashy trash}

\begin{bluetext}
\proof
For $t \le h$, let $V_t = \tilde{v}^{k,\epsilon}(t,p,\tilde{E}^{k,\epsilon}_t) - v^{k,\epsilon}(t,p,\tilde{E}^{k,\epsilon}_t) $.
Applying Ito's formula, we compute
\begin{align*}
V_t = V_0 - \int_0^t\left(\partial_tv^{k,\epsilon}(s,p,\tilde{E}^{k,\epsilon}_s) + \mu(\tilde{Y}^{k,\epsilon}_s,p)\partial_e v^{k,\epsilon}(s,p,\tilde{E}^{k,\epsilon}_s) + \frac12\epsilon^2\partial^2_{ee}v^{k,\epsilon}(s,p,\tilde{E}^{k,\epsilon}_s) \right)\ud s + M^{k,\epsilon}_t,
\end{align*}
where $M$ is a square-integrable martingale.\\
From the PDE \eqref{value function pde} satisfied by $v^{k,\epsilon}$, we get
\begin{align*}
V_t = V_0 + \int_0^t \left( \cL^pv^{k,\epsilon}(s,p,\tilde{E}^{k,\epsilon}_s) - (
 \mu(\tilde{Y}^{k,\epsilon}_s,p)  - \mu(v^{k,\epsilon}(s,p,\tilde{E}^{k,\epsilon}_s),p))\partial_e v^{k,\epsilon}(s,p,\tilde{E}^{k,\epsilon}_s) \right) \ud s + M^{k,\epsilon}_t
\end{align*}
Introduce
\begin{align}
c_s := \int_0^1\partial_y \mu(v^{k,\epsilon}(s,p,\tilde{E}^{k,\epsilon}_s) + \lambda V_s) \ud \lambda \le 0
\end{align}
Thus, the previous equality reads
\begin{align*}
V_t = V_0 + \int_0^t \left( \cL^pv^{k,\epsilon}(s,p,\tilde{E}^{k,\epsilon}_s) - c_s V_s \partial_e v^{k,\epsilon}(s,p,\tilde{E}^{k,\epsilon}_s) \right) \ud s + M^{k,\epsilon}_t
\end{align*}
We then compute, setting $\cE_t = e^{\int_0^t c_s \partial_e v^{k,\epsilon}(s,p,\tilde{E}^{k,\epsilon}_s)  \ud s} \in [0,1]$, $t \le h$,
\begin{align}
\cE_t V_t = V_0 + \int_0^t \cE_s \cL^pv^{k,\epsilon}(s,p,\tilde{E}^{k,\epsilon}_s)\ud s  + N^{k,\epsilon}_t
\end{align}
In particular, we get
\begin{align}\label{eq almost conclusion}
|V_0| \le \esp{|V_h| +\int_0^h|\cL^pv^{k,\epsilon}(s,p,\tilde{E}^{k,\epsilon}_s)|\ud s}
\end{align}
From \textcolor{red}{assumption \eqref{eq ass second order controlled}}, we have 
\begin{align} \label{eq controlling Lp}
\int_0^h|\cL^pv^{k,\epsilon}(s,p,\tilde{E}^{k,\epsilon}_s)|\ud s \le Ch.
\end{align}
Moreover, we observe
\begin{align*}
V_h &= \bar{v}^{k,\epsilon}(0,p,\tilde{E}^{k,\epsilon}_h) - \psi^k(p,\tilde{E}^{k,\epsilon}_h)
\\
&= \esp{\psi^k(P^\epsilon_h,\tilde{E}^{k,\epsilon}_h)-\psi^k(p,\tilde{E}^{k,\epsilon}_h)}
\end{align*}
leading to $\esp{|V_h|} \le C \esp{|P^\epsilon_h-p|}\le C\sqrt{h}$. 
Combining the previous inequality with \eqref{eq almost conclusion} and  \eqref{eq controlling Lp} concludes the proof.
\eproof
\end{bluetext}

\begin{magetext}
\begin{Remark}
dans la preuve on a figé $p$, ce qui fait apparaitre les derivées  en $p$ de $v^{k,\epsilon}$. On aurait pu faire apparaitre les derivees de $\tilde{v}^{k,\epsilon}$ en $p$ en utilisant comme definition de $V$, $V_t = \tilde{v}^{k,\epsilon}(t,P^\epsilon,\tilde{E}^{k,\epsilon}_t) - v^{k,\epsilon}(t,P^\epsilon_t,\tilde{E}^{k,\epsilon}_t)$. le point important etant que dans la différence des $\mu$ le même processus soit dans la $p$-variable...
\end{Remark}
\end{magetext}



\subsubsection{Truncation error}
this is given by 
$\eta(t_i,p,e)$ which should somehow represent the error on the interval $[t_i,t_{i+1}]$
\\
\textcolor{red}{the study of this truncation error is not finished...}

\begin{bluetext}
Let us define $V^{p,e}_s := v(s,P_s,\tilde{E}^{p,e}_s)$, $\tilde{V}^{p,e}_s=\tilde{v}(s,p,\tilde{E}^{p,e}_s)$,
\begin{align}
U^{p,e}_s = \tilde{v}(s,p,\tilde{E}^{p,e}_s) - v(s,P_s,\tilde{E}^{p,e}_s)\,,\; 0 \le s \le h\,, p \in \R, e \in \R,
\end{align}
where
\begin{align}
\tilde{E}^{p,e}_s = e  - \int_0^s f(\tilde{V}_t) \ud t
\end{align}
which is the characteristic associated to \eqref{eq tr op} (OK via carmona-delarue).
Note that one can always add some noise to perform the computation below...\\
First let us note that by the property of the characteristics: $\tilde{v}(s,p,\tilde{E}^{p,e}_s) = cste$ for all $0 \le s \le h$ and applying Itô's formula to the second term, we get
\begin{align}
U_t = U_0 - \int_{0}^t  \left( \partial_t v(s,P_s, \tilde{E}^{p,e}_s) + \frac12 \partial^2_{pp} v(s,P_s, \tilde{E}^{p,e}_s) -f(\tilde{V}_s)\partial_e v(s,P_s, \tilde{E}^{p,e}_s) \right)\ud s + M_t
\end{align}
Using the PDE \eqref{main eq} satisfied by $v$, we get
\begin{align}
U_t = U_0 - \int_{0}^t  \left( f({v}(s,P_s, \tilde{E}^{p,e}_s)) -f(\tilde{v}(s,p, \tilde{E}^{p,e}_s))\right)\partial_e v(s,P_s, \tilde{E}^{p,e}_s) \ud s + M_t
\end{align}
Denoting
$
c^f_s := \int_0^1 f'(V_s + \lambda U_s) \ud \lambda
$,
 we have
\begin{align}
U_t = U_0 + \int_{0}^t  c^f_s U_s \partial_e v(s,P_s, \tilde{E}^{p,e}_s) \ud s + M_t
\end{align}
Introducing $\bar{U}_t = e^{-\int_0^tc^f_s \partial_e v(s,P_s, \tilde{E}^{p,e}_s) \ud s} U_t$, we obtain
\begin{align}
U_0 = \esp{e^{-\int_0^hc^f_s \partial_e v(s,P_s, \tilde{E}^{p,e}_s) \ud s} U_h}
\end{align}
\end{bluetext}
%\input{splitting}

\section{Classical approach revisited}
To simplify the notation, we introduce $\check{v}(t_{i+1},p,e) := \esp{\tilde{v}(t_{i+1},P^{t_i,p}_{t_{i+1}},e)}=\cD_h[\tilde{v}(t_{i+1},\cdot)](p,e)$ (the diffusion part only). We recall also that $\tilde{v}$ is obtained on $[t_i,t_{i+1})$ via the transport equation, in particular $\tilde{v}(t_i,\cdot) = \cT_h[\check{v}(t_{i+1},\cdot)]$.

\begin{Proposition}
In the setting, introduced in Section 1, we have
\begin{align}
|\tilde{v}(0,p,e)-{v}(0,p,e)| \le \sum_{i=0}^{n-1} \esp{|\EFp{t_i}{\cR(t_i,P_{t_i},\tilde{E}_{t_i})}|}
\end{align}
where $\cR$ is defined below in equation \eqref{eq de remainder}.
\end{Proposition}
\textcolor{magenta}
{
$\Longrightarrow$ C'est pour l'étude de $\cR$ (erreur de troncation) qu'on va avoir besoin de la régularité Lipschitz de $v$ en $e$ et de beaucoup de régularité sur $\partial_{pp}v$ aussi $p$,$t$ et $e$ ...
}


\begin{bluetext}
\proof
1. at step $i$:
For $t_i \le s <t_{i+1}$, let us define $V^{p,e}_s := v(s,p,\tilde{E}^{p,e}_s)$, $\tilde{V}^{p,e}_s=\tilde{v}(s,p,\tilde{E}^{p,e}_s)$,
\begin{align}
U^{p,e}_s = \tilde{V}^{p,e}_s- V^{p,e}_s\,,\; t_i \le s < t_{i+1}\,, p \in \R, e \in \R,
\end{align}
where
\begin{align}
\tilde{E}^{p,e}_s = e  - \int_{t_i}^s f(\tilde{V}^{p,e}_t) \ud t
\end{align}
which is the characteristic associated to \eqref{eq tr op} (OK via carmona-delarue).
(Note that one can always add some noise to perform the computation below if needed...)\\
First let us note that by the property of the characteristics: $\tilde{v}(s,p,\tilde{E}^{p,e}_s) = cste$ for all $t_i \le t < t_{i+1}$ and applying the chain rule of calculus to the second term, we get
\begin{align}
U^{p,e}_{t} = U^{p,e}_{t_i} - \int_{0}^t  \left( \partial_t v(s,p, \tilde{E}^{p,e}_s)  -f(\tilde{V}_s)\partial_e v(s,p, \tilde{E}^{p,e}_s) \right)\ud s 
\end{align}
Using the PDE \eqref{main eq} satisfied by $v$, we get
\begin{align}
U^{p,e}_t = U^{p,e}_{t_i} - \int_{t_i}^t  \left( (f({V}^{p,e}_s) -f(\tilde{V}^{p,e}_s))\partial_e v(s,p, \tilde{E}^{p,e}_s) - \frac12\partial_{pp}v(s,p,\tilde{E}^{p,e}_s)\right)\ud s 
\end{align}
Denoting
$
c^{p,e}_s := \int_0^1 f'(V_s + \lambda U_s) \ud \lambda
$,
 we have
\begin{align}
U^{p,e}_t = U^{p,e}_{t_i} + \int_{t_i}^t  c^{p,e}_s U^{p,e}_s \partial_e v(s,p, \tilde{E}^{p,e}_s) \ud s + 
\frac12\int_{t_i}^t \partial_{pp}v(s,p,\tilde{E}^{p,e}_s) \ud s 
\end{align}
Introducing $\bar{U}^{p,e}_t = \cE^{t_i,p,e}_t  U^{p,e}_t$ with $\cE^{t_i,p,e}_t := e^{-\int_{t_i}^tc^{p,e}_s \partial_e v(s,p, \tilde{E}^{p,e}_s) \ud s} $ and applying Ito's formula, we obtain
\begin{align}
U^{p,e}_{t_{i}} = \cE^{t_i,p,e}_{t_{i+1}} U^{p,e}_{t_{i+1}-} - \frac12 \int_{t_i}^{t_{i+1}}\cE^{t_i,p,e}_s\partial_{pp}v(s,p,\tilde{E}^{p,e}_s) \ud s
\end{align}
Now,
\begin{align}
U^{p,e}_{t_{i+1}-} = \tilde{V}^{p,e}_{t_{i+1}}- V^{p,e}_{t_{i+1}} &= \check{v}(t_{i+1},p,\tilde{E}^{p,e}_{t_{i+1}}) - v(t_{i+1},p,\tilde{E}^{p,e}_{t_{i+1}})
\\
&= \tilde{v}(t_{i+1},P^{p,t_i}_{t_{i+1}},\tilde{E}_{t_{i+1}}) + \Delta \tilde{M}^{p,e}_i -v(t_{i+1},P^{p,t_i}_{t_{i+1}},\tilde{E}_{t_{i+1}}) 
\\& \quad + v(t_{i+1},P^{p,t_i}_{t_{i+1}},\tilde{E}_{t_{i+1}}) - v(t_{i+1},p,\tilde{E}_{t_{i+1}})
\end{align}
We compute
\begin{align}
v(t_{i+1},P^{p,t_i}_{t_{i+1}},\tilde{E}_{t_{i+1}}) - v(t_{i+1},p,\tilde{E}_{t_{i+1}})= \frac12 \int_{t_i}^{t_{i+1}} \partial_{pp}v(t_{i+1},P_s,\tilde{E}^{p,e}_{t_{i+1}}) \ud s  + \Delta M^{p,e}_i\;.
\end{align}
Thus,
\begin{align}
U^{p,e}_{t_i} &= \cE^{t_i,p,e}_{t_{i+1}} U^{p,e}_{t_{i+1}} + \cR(t_i,p,e)
+\cE^{t_i,p,e}_{t_{i+1}} (\Delta M^{p,e}_i+\Delta \tilde{M}^{p,e}_i)
\end{align}
where
\begin{align}
 \cR(t_i,p,e) &= \frac12 \int_{t_i}^{t_{i+1}}\left( \cE^{t_i,p,e}_{t_{i+1}} \partial_{pp}v(t_{i+1},P^{t_i,p}_s,\tilde{E}^{p,e}_{t_{i+1}}) - \cE^{t_i,p,e}_{s} \partial_{pp}v(s,p,\tilde{E}^{p,e}_s) \right) \ud s 
 \label{eq de remainder}
 \\
  \cM(t_i,p,e) &=  \cE^{t_i,p,e}_{t_{i+1}} (\Delta M^{p,e}_i+\Delta \tilde{M}^{p,e}_i)
\end{align}
2. On $[0,T]$, we define $P_t = p + W_t$ and  $\tilde{E}$, recursively by
\begin{align}
\tilde{E}_{t} = \tilde{E}_{t_i} -\int_{t_i}^{t}f(\tilde{v}(s,P_{t_i},\tilde{E}_s) )\ud s
\end{align}
for  $t \in [t_i,t_{i+1})$ and $E_0 = e$. In this context, we also define
\begin{align}
U_{t_i} = \tilde{v}(t_i,P_{t_i},\tilde{E}_{t_i})-{v}(t_i,P_{t_i},\tilde{E}_{t_i})\;.
\end{align}
From the previous step, we have
\begin{align*}
|U_{t_i}| & \le \cE^{t_i,P_{t_i},\tilde{E_{t_i}}}_{t_{i+1}} \EFp{t_i}{|U_{t_{i+1}}| }+ |\EFp{t_i}{\cR(t_i,P_{t_i},\tilde{E}_{t_i})}|
\\
& \le \EFp{t_i}{|U_{t_{i+1}}| }+ |\EFp{t_i}{\cR(t_i,P_{t_i},\tilde{E}_{t_i})}|
\end{align*}
The proof is concluded by iterating on $i$.
\end{bluetext}

